Reinforcement Learning Assisted Load Test Generation for E-Commerce Applications

Background: End-user satisfaction is not only dependent on the correct functioning of the software systems but is also heavily dependent on how well those functions are performed. Therefore, performance testing plays a critical role in making sure that the system responsively performs the indented functionality. Load test generation is a crucial activity in performance testing. Existing approaches for load test generation require expertise in performance modeling, or they are dependent on the system model or the source code. Aim: This thesis aims to propose and evaluate a model-free learning-based approach for load test generation, which doesn't require access to the system models or source code. Method: In this thesis, we treated the problem of optimal load test generation as a reinforcement learning (RL) problem. We proposed two RL-based approaches using q-learning and deep q-network for load test generation. In addition, we demonstrated the applicability of our tester agents on a real-world software system. Finally, we conducted an experiment to compare the efficiency of our proposed approaches to a random load test generation approach and a baseline approach. Results: Results from the experiment show that the RL-based approaches learned to generate effective workloads with smaller sizes and in fewer steps. The proposed approaches led to higher efficiency than the random and baseline approaches. Conclusion: Based on our findings, we conclude that RL-based agents can be used for load test generation, and they act more efficiently than the random and baseline approaches.

==> etics.tex <==
\section{Ethical and Societal Considerations}

I f\"{o}rst hand avser vi med ”etik” h\"{a}r forskningsetiska fr\r{a}gor. Inneb\"{a}r ditt val av fr\r{a}gest\"{a}llning eller metod n\r{a}got forskningsetiskt st\"{a}llningstagande? Om du till exempel intervjuar personer f\"{o}r ditt arbete, kan du garantera dessa anonymitet och p\r{a} vilket s\"{a}tt anv\"{a}nder du den information du f\r{a}r av dem? Finns det andra etiska aspekter att beakta i arbetet? Kan det finnas etiska aspekter p\r{a} resultatet av ditt arbete? Du b\"{o}r tydligt ange om du anser att ditt arbete inte inneh\r{a}ller n\r{a}gra forskningsetiska fr\r{a}gor. 

Du ska ocks\r{a} kritiskt granska och analysera ditt arbete med h\"{a}nsyn till samh\"{a}lleliga aspekter. H\"{a}r kan du till exempel diskutera hur ditt arbete f\"{o}rh\r{a}ller sig till m\r{a}l som ekonomisk, social och ekologiskt h\r{a}llbar utveckling. Det kan ocks\r{a} finnas juridiska och politiska aspekter p\r{a} ditt arbete. 


==> outcome.tex <==
\section{Outcome and Timetable \textcolor{red}{(This page should be deleted)}}\label{outcome}

\subsection{Outcome }
Our technical contribution in this thesis is the implementation of an RL based agent, that will learn and reuse the optimal policy for load generation. We aim to evaluate the applicability and effectiveness of our approach using a case study research method. Our contributions will add to the body of knowledge by reporting relevant quantitative results of the application of RL based approach for load testing.

\subsection{Timetable}

\vspace{5mm}

\begin{center}
\begin{tabular}{ | m{23em} | m{8em} | } 
\hline
\textbf{Activity} & \textbf{Date}\\
\hline
Start date & January 20, 2020 \\ 
\hline
Status and planning report submission & February 09, 2020 \\ 
\hline
Status and planning seminar & February 12, 2020 \\
\hline
RL load tester detailed architecture (design delivery) & March 1, 2020 \\
\hline
RL load tester implementation & March 15, 2020 \\
\hline
SUT and load generator tool (Apache JMeter) setup & April 1, 2020 \\
\hline
Experimental evaluation of the proposed approach & May 1, 2020 \\
\hline
Final Report submission & May 20, 2020 \\
\hline
Opponent ship report submission & June 2, 2020 \\ 
\hline
Presentation dates & June 4-5, 2020 \\
\hline
\end{tabular}
\end{center}


